Channel-Temporal Attention for First-Person Video Domain Adaptation

Unsupervised Domain Adaptation (UDA) can transfer knowledge from labeled source data to unlabeled target data of the same categories. However, UDA for first-person action recognition is an under-explored problem, with lack of datasets and limited consideration of first-person video characteristics. This paper focuses on addressing this problem. Firstly, we propose two small-scale first-person video domain adaptation datasets: ADL$_{small}$ and GTEA-KITCHEN. Secondly, we introduce channel-temporal attention blocks to capture the channel-wise and temporal-wise relationships and model their inter-dependencies important to first-person vision. Finally, we propose a Channel-Temporal Attention Network (CTAN) to integrate these blocks into existing architectures. CTAN outperforms baselines on the two proposed datasets and one existing dataset EPIC$_{cvpr20}$.

==> test.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}

% \usepackage{iccv}
% \usepackage{times}
% \usepackage{epsfig}
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}

% \usepackage{color}
% \usepackage{subfigure}
% \usepackage{algorithm, algorithmic}
% \usepackage{cite}
% \usepackage{multirow}

% \usepackage[utf8]{inputenc}
% \usepackage{textcomp}
% \usepackage{booktabs}  % for prettier tables
% \usepackage{array} % for raggedleft tabular parapgrahs
% \usepackage{lipsum} % HC for table alignment  
% \usepackage{enumitem} % for no left margin in itemize
% \usepackage{placeins}
% \usepackage{diagbox}


% % Include other packages here, before hyperref.

% % If you comment hyperref and then uncomment it, you should delete
% % egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% % run, let it finish, and you should be clear).
% \usepackage[pagebackref=true,breaklinks=true,letterpaper=true,colorlinks,bookmarks=false]{hyperref}

% \iccvfinalcopy % *** Uncomment this line for the final submission

% \def\iccvPaperID{9197} % *** Enter the ICCV Paper ID here
% \def\httilde{\mbox{\tt\raisebox{-.5ex}{\symbol{126}}}}

% % Pages are numbered in submission mode, and unnumbered in camera-ready
% \ificcvfinal\pagestyle{empty}\fi

% \begin{document}

%%%%%%%%% TITLE
\title{Channel-Temporal Attention for First-Person Video Domain Adaptation}
% \title{Multi-Adversarial Channel-Temporal Attention for First-Person Video Domain Adaptation}
\author{Xianyuan Liu\textsuperscript{\rm 1,2,3}, 
Shuo Zhou\textsuperscript{\rm 3},
Tao Lei\textsuperscript{\rm 1,2},
Haiping Lu\textsuperscript{\rm 3}\\
\textsuperscript{\rm 1}Institute of Optical and Electronics, Chinese Academy of Sciences, China\\
\textsuperscript{\rm 2}University of Chinese Academy of Sciences, China\\
\textsuperscript{\rm 3}University of Sheffield, United Kingdom\\
\{xianyuan.liu, szhou20, h.lu\}@sheffield.ac.uk, taoleiyan@ioe.ac.cn
}

% \author{First Author\\
% Institution1\\
% Institution1 address\\
% {\tt\small firstauthor@i1.org}
% For a paper whose authors are all at the same institution,
% omit the following lines up until the closing ``}''.
% Additional authors and addresses can be added with ``\and'',
% just like the second author.
% To save space, use either the email address or home page, not both
% \and
% Second Author\\
% Institution2\\
% First line of institution2 address\\
% {\tt\small secondauthor@i2.org}
% }

\maketitle
% Remove page # from the first page of camera-ready.
\ificcvfinal\thispagestyle{empty}\fi

%%%%%%%%% ABSTRACT
\begin{abstract}
% \input{sections/abstract}
Unsupervised Domain Adaptation (UDA) can transfer knowledge from labeled source data to unlabeled target data of the same categories. However, UDA for first-person action recognition is an under-explored problem, with lack of datasets and limited consideration of first-person video characteristics. This paper focuses on addressing this problem. Firstly, we propose two small-scale first-person video domain adaptation datasets: ADL$_{small}$ and GTEA-KITCHEN. Secondly, we introduce channel-temporal attention blocks to capture the channel-wise and temporal-wise relationships and model their inter-dependencies important to first-person vision. Finally, we propose a 
Channel-Temporal Attention Network (CTAN) to integrate these blocks into existing architectures. CTAN outperforms baselines on the two proposed datasets and one existing dataset EPIC$_{cvpr20}$.
% Unsupervised Domain Adaptation (UDA) can transfer knowledge from labeled source data to unlabeled target data where annotation is not available and impractical. % (to (reduce the need of annotation.)).
% However, few attempts have been devoted to UDA for first-person action recognition due to the lack of datasets,
% % and the special characteristics.
% resulting in few exploration in the special characteristics of first-person video for UDA. This paper focuses on addressing this problem. First, we propose two small-scale video domain adaptation datasets: ADL$_{small}$ and GTEA-KITCHEN. Second, we introduce channel-temporal attention blocks to capture the channel-wise and temporal-wise relationships and model their inter-dependencies. Finally, we propose a 
% % Multi-Adversarial 
% Channel-Temporal Attention Network (CTAN) to integrate these blocks into the existing architecture. Our network outperforms the baselines on our proposed datasets and EPIC$_{cvpr20}$.
\end{abstract}

%%%%%%%%% BODY TEXT
\section{Introduction}

Video-based action recognition is a challenging computer vision problem. Great progress has been made on several benchmark datasets \cite{Kuehne11,soomro2012ucf101,kay2017kinetics,Damen2018EPICKITCHENS} using architectures based on Convolutional Neural Networks (CNNs) \cite{Feichtenhofer_2016_CVPR,Carreira_2017_CVPR,tran2018closer,8454294}. However, it remains a major obstacle to generalize models learned on one domain to another domain due to the distribution mismatch between them, i.e., the \textit{domain shift}. Moreover, domain discrepancy not only exists between different datasets but also between different videos in the same dataset, e.g. as shown in Table .

{\small
\bibliographystyle{ieee_fullname}
\bibliography{ms.bib}
}

% \end{document}
